LIGOs Quantum Response to Squeezed States

Gravitational Wave interferometers achieve their profound sensitivity by combining a Michelson interferometer with optical cavities, suspended masses, and now, squeezed quantum states of light. These states modify the measurement process of the LIGO, VIRGO and GEO600 interferometers to reduce the quantum noise that masks astrophysical signals; thus, improvements to squeezing are essential to further expand our gravitational view of the universe. Further reducing quantum noise will require both lowering decoherence from losses as well more sophisticated manipulations to counter the quantum back-action from radiation pressure. Both tasks require fully understanding the physical interactions between squeezed light and the many components of km-scale interferometers. To this end, data from both LIGO observatories in observing run three are expressed using frequency-dependent metrics to analyze each detector's quantum response to squeezed states. The response metrics are derived and used to concisely describe physical mechanisms behind squeezing's simultaneous interaction with transverse-mode selective optical cavities and the quantum radiation pressure noise of suspended mirrors. These metrics and related analysis are broadly applicable for cavity-enhanced optomechanics experiments that incorporate external squeezing, and -- for the first time -- give physical descriptions of every feature so far observed in the quantum noise of the LIGO detectors.

==> FreqLoss_arxiv/authors.tex <==
\author{L.~McCuller}
\email{lee.mcculler@ligo.org}  %lee.mcculler
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{S.~E.~Dwyer}  %sheila.dwyer
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}

\author{A.~C.~Green}
\affiliation{University of Florida, Gainesville, FL 32611, USA}

\author{Haocun~Yu}  %haocun.yu
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{L.~Barsotti}  %lisa.barsotti
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{C.~D.~Blair}  %carl.blair
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}

\author{D.~D.~Brown}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}


\author{A.~Effler}  %anamaria.effler
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}

\author{M.~Evans}  %matthew.evans
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{A.~Fernandez-Galiana}  %alvaro.fernandez-galiana
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{P.~Fritschel}  %peter.fritschel
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{V.~V.~Frolov}  %valery.frolov
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}

\author{N.~Kijbunchoo}  %nutsinee.kijbunchoo
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}

\author{G.~L.~Mansell}  %georgia.mansell
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}

\author{F.~Matichard}  %fabrice.matichard
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{N.~Mavalvala}  %nergis.mavalvala
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{D.~E.~McClelland}  %david.mcclelland
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}

\author{T.~McRae}  %terry.mcrae
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}

\author{A.~Mullavey}  %adam.mullavey
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}

\author{D.~Sigg}  %daniel.sigg
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}

\author{B.~J.~J.~Slagmolen}  %bram.slagmolen
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}

\author{M.~Tse}  %maggie.tse
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{T.~Vo}  %thomas.vo
\affiliation{Syracuse University, Syracuse, NY 13244, USA}

\author{R.~L.~Ward}
\affiliation{OzGrav, Australian National University, Canberra,
  Australian Capital Territory 0200, Australia} 

\author{C.~Whittle}%chris.whittle
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

% Detector author list from LIGO-M2000148-v4, less the squeezer authors above
\author{R.~Abbott}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~Adams}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{R.~X.~Adhikari}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Ananyeva}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~Appert}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.~Arai}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~S.~Areeda}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{Y.~Asali}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{S.~M.~Aston}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{C.~Austin}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{A.~M.~Baer}
\affiliation{Christopher Newport University, Newport News, VA 23606, USA}
\author{M.~Ball}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{S.~W.~Ballmer}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{S.~Banagiri}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}
\author{D.~Barker}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~Bartlett}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{B.~K.~Berger}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{J.~Betzwieser}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~Bhattacharjee}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\author{G.~Billingsley}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{S.~Biscans}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~M.~Blair}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{N.~Bode}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{P.~Booker}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{R.~Bork}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Bramley}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~F.~Brooks}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Buikema}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{C.~Cahillane}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.~C.~Cannon}
\affiliation{RESCEU, University of Tokyo, Tokyo, 113-0033, Japan.}
\author{X.~Chen}
\affiliation{OzGrav, University of Western Australia, Crawley, Western Australia 6009, Australia}
\author{A.~A.~Ciobanu}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{F.~Clara}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{C.~M.~Compton}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~J.~Cooper}
\affiliation{University of Birmingham, Birmingham B15 2TT, UK}
\author{K.~R.~Corley}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{S.~T.~Countryman}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{P.~B.~Covas}
\affiliation{Universitat de les Illes Balears, IAC3---IEEC, E-07122 Palma de Mallorca, Spain}
\author{D.~C.~Coyne}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{L.~E.~H.~Datrier}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{D.~Davis}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{C.~Di~Fronzo}
\affiliation{University of Birmingham, Birmingham B15 2TT, UK}
\author{K.~L.~Dooley}
\affiliation{Cardiff University, Cardiff CF24 3AA, UK}
\affiliation{The University of Mississippi, University, MS 38677, USA}
\author{J.~C.~Driggers}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{T.~Etzel}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{T.~M.~Evans}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~Feicht}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{P.~Fulda}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Fyffe}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~A.~Giaime}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{K.~D.~Giardina}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{P.~Godwin}
\affiliation{The Pennsylvania State University, University Park, PA 16802, USA}
\author{E.~Goetz}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\affiliation{Missouri University of Science and Technology, Rolla, MO 65409, USA}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{S.~Gras}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{C.~Gray}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{R.~Gray}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{E.~K.~Gustafson}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Gustafson}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{J.~Hanks}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~Hanson}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{T.~Hardwick}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{R.~K.~Hasskew}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{M.~C.~Heintze}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~F.~Helmling-Cornell}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{N.~A.~Holland}
\affiliation{OzGrav, Australian National University, Canberra, Australian Capital Territory 0200, Australia}
\author{J.~D.~Jones}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~Kandhasamy}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{S.~Karki}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{M.~Kasprzack}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.~Kawabe}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{P.~J.~King}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~S.~Kissel}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{Rahul~Kumar}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Landry}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{B.~B.~Lane}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{B.~Lantz}
\affiliation{Stanford University, Stanford, CA 94305, USA}
\author{M.~Laxen}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{Y.~K.~Lecoeuche}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~Leviton}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{J.~Liu}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{M.~Lormand}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~P.~Lundgren}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{R.~Macas}
\affiliation{Cardiff University, Cardiff CF24 3AA, UK}
\author{M.~MacInnis}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{D.~M.~Macleod}
\affiliation{Cardiff University, Cardiff CF24 3AA, UK}
\author{S.~M\'arka}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{Z.~M\'arka}
\affiliation{Columbia University, New York, NY 10027, USA}
\author{D.~V.~Martynov}
\affiliation{University of Birmingham, Birmingham B15 2TT, UK}
\author{K.~Mason}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{T.~J.~Massinger}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{R.~McCarthy}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{S.~McCormick}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~McIver}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{University of British Columbia, Vancouver, BC V6T 1Z4, Canada}
\author{G.~Mendell}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{K.~Merfeld}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{E.~L.~Merilh}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{F.~Meylahn}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\author{T.~Mistry}
\affiliation{The University of Sheffield, Sheffield S10 2TN, UK}
\author{R.~Mittleman}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{G.~Moreno}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{C.~M.~Mow-Lowry}
\affiliation{University of Birmingham, Birmingham B15 2TT, UK}
\author{S.~Mozzon}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{T.~J.~N.~Nelson}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{P.~Nguyen}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{L.~K.~Nuttall}
\affiliation{University of Portsmouth, Portsmouth, PO1 3FX, UK}
\author{J.~Oberling}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{Richard~J.~Oram}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{C.~Osthelder}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{D.~J.~Ottaway}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{H.~Overmier}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{J.~R.~Palamos}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{W.~Parker}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\affiliation{Southern University and A\&M College, Baton Rouge, LA 70813, USA}
\author{E.~Payne}
\affiliation{OzGrav, School of Physics \& Astronomy, Monash University, Clayton 3800, Victoria, Australia}
\author{A.~Pele}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{R.~Penhorwood}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{C.~J.~Perez}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Pirello}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{H.~Radkins}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{K.~E.~Ramirez}
\affiliation{The University of Texas Rio Grande Valley, Brownsville, TX 78520, USA}
\author{J.~W.~Richardson}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{K.~Riles}
\affiliation{University of Michigan, Ann Arbor, MI 48109, USA}
\author{N.~A.~Robertson}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{J.~G.~Rollins}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{C.~L.~Romel}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~H.~Romie}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{M.~P.~Ross}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{K.~Ryan}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{T.~Sadecki}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{E.~J.~Sanchez}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{L.~E.~Sanchez}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{T.~R.~Saravanan}
\affiliation{Inter-University Centre for Astronomy and Astrophysics, Pune 411007, India}
\author{R.~L.~Savage}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{D.~Schaetzl}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Schnabel}
\affiliation{Universit\"at Hamburg, D-22761 Hamburg, Germany}
\author{R.~M.~S.~Schofield}
\affiliation{University of Oregon, Eugene, OR 97403, USA}
\author{E.~Schwartz}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{D.~Sellers}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{T.~Shaffer}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{J.~R.~Smith}
\affiliation{California State University Fullerton, Fullerton, CA 92831, USA}
\author{S.~Soni}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{B.~Sorazu}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{A.~P.~Spencer}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{K.~A.~Strain}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{L.~Sun}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~J.~Szczepa\'nczyk}
\affiliation{University of Florida, Gainesville, FL 32611, USA}
\author{M.~Thomas}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{P.~Thomas}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{K.~A.~Thorne}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{K.~Toland}
\affiliation{SUPA, University of Glasgow, Glasgow G12 8QQ, UK}
\author{C.~I.~Torrie}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{G.~Traylor}
\affiliation{LIGO Livingston Observatory, Livingston, LA 70754, USA}
\author{A.~L.~Urban}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{G.~Vajente}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{G.~Valdes}
\affiliation{Louisiana State University, Baton Rouge, LA 70803, USA}
\author{D.~C.~Vander-Hyde}
\affiliation{Syracuse University, Syracuse, NY 13244, USA}
\author{P.~J.~Veitch}
\affiliation{OzGrav, University of Adelaide, Adelaide, South Australia 5005, Australia}
\author{K.~Venkateswara}
\affiliation{University of Washington, Seattle, WA 98195, USA}
\author{G.~Venugopalan}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~D.~Viets}
\affiliation{Concordia University Wisconsin, 2800 N Lake Shore Dr, Mequon, WI 53097, USA}
\author{C.~Vorvick}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{M.~Wade}
\affiliation{Kenyon College, Gambier, OH 43022, USA}
\author{J.~Warner}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{B.~Weaver}
\affiliation{LIGO Hanford Observatory, Richland, WA 99352, USA}
\author{R.~Weiss}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{B.~Willke}
\affiliation{Leibniz Universit\"at Hannover, D-30167 Hannover, Germany}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute), D-30167 Hannover, Germany}
\author{C.~C.~Wipf}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{L.~Xiao}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{H.~Yamamoto}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Hang~Yu}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\author{L.~Zhang}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{M.~E.~Zucker}
\affiliation{LIGO, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}
\author{J.~Zweizig}
\affiliation{LIGO, California Institute of Technology, Pasadena, CA 91125, USA}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "fdep_main.tex"
%%% End: 
